An Efficient Nonlinear Acceleration method that Exploits Symmetry of the Hessian

Nonlinear acceleration methods are powerful techniques to speed up fixed-point iterations. However, many acceleration methods require storing a large number of previous iterates and this can become impractical if computational resources are limited. In this paper, we propose a nonlinear Truncated Generalized Conjugate Residual method (nlTGCR) whose goal is to exploit the symmetry of the Hessian to reduce memory usage. The proposed method can be interpreted as either an inexact Newton or a quasi-Newton method. We show that, with the help of global strategies like residual check techniques, nlTGCR can converge globally for general nonlinear problems and that under mild conditions, nlTGCR is able to achieve superlinear convergence. We further analyze the convergence of nlTGCR in a stochastic setting. Numerical results demonstrate the superiority of nlTGCR when compared with several other competitive baseline approaches on a few problems. Our code will be available in the future.

==> AA2_ver_saad.tex <==
\section{Exploiting symmetry}
In the following, we specifically consider the case where the nonlinear mapping
$f$ is the gradient of some
objective function $\phi(x):\mathbb{R}^n\rightarrow\mathbb{R}$ to be minimized, i.e., $$f(x) = \nabla \phi(x). $$
In this situation the Jacobian of $f$ becomes $\nabla^2 \phi$  the Hessian of $\phi$. An obvious observation here is that the symmetry of the Hessian is not taken into account in the approximate inverse Hessian update formula
  \nref{eq:msec}. This has been considered
  in the literature (very) recently, see for example,
  \cite{Boutet2020,scieur21a,Boutet2021}.  In a 1983 report, Schnabel
  \cite{Schnabel83} showed that the matrix $G_j$ obtained by a multi-secant method
  that satisfies the secant condition \nref{eq:mscond} is symmetric iff the
  matrix $\XX_j^T \FF_j$ is symmetric. It is possible to explicitly force
  symmetry by employing generalizations of the symmetric versions of
  Broyden-type methods. Thus, the authors of \cite{Boutet2020,Boutet2021}
  recently developed a multisecant version of the Powell Symmetric Broyden (PSB)
  update due to Powell \cite{Powell70} while the article \cite{scieur21a}
  proposed a symmetric multisecant method based on the popular
  Broyden-Fletcher-Goldfarb-Shanno (BFGS) approach as well as the
  Davidon-Fletcher-Powell (DFP) update. However, there are a number of  issues with the symmetric versions of multisecant updates some of which are  discussed in~\cite{scieur21a}. 
  
 We observe that when we are close to the limit, the condition
   $\XX_j^T \FF_j =  \FF_j^T \XX_j $ is nearly satisfied for AA.
  This is because if $x_*$ is the limit with $f(x_*) = 0$ we can write
  \begin{eqnarray*}
    f(x_k) - f(x_{k-1}) &=& 
    [ f(x_k) - f(x_*)] - [ f(x_{k-1}) - f(x_*)]\approx \nabla^2 \phi(x_*) ( x_k \ - \ x_{k-1}) . 
                                      %%&\approx&  \nabla^2 f(x_*) ( x_k \ - \ x_{k-1}) .
  \end{eqnarray*}
  This translates to $\FF_j \approx  \nabla^2 \phi(x_*) \XX_j $
  from which it follows that
  $ \XX_j^T \FF_j \approx  \XX_j^T   \nabla^2 \phi(x_*) \XX_j $ which is a
  symmetric matrix under mild smoothness conditions on $\phi$.
  Therefore, the issue of symmetry can be mitigated if we are able develop nonlinear acceleration methods that take advantage of 
  near-symmetry.  

  
  \subsection{The linear case: Truncated GCR (\methodName)}
  %We first consider the quadratic function
  %$\phi_q(x) \equiv \half \| b - A x\|_2^2 $.  Solving $\nabla \phi_q = 0$ is
  %equivalent to solving the linear system $Ax=b$.  
  We first consider solving the linear system $Ax=b$ with a general matrix
  $A$. Generalized
  Conjugate Residual (GCR) algorithm, see, e.g., \cite{Saad-book2}, solves
  this linear system by
  building a sequence of search directions $p_i$, for $i=0, \cdots, j$ at step $j$
  so that the vectors  $A p_i$ are orthogonal to each other.
 With this property it is easy to generate iterates
 that minimize the residual at each step,
  and this leads to GCR,  see \cite[pp 195-196]{Saad-book2} for details.

Next we will make two changes to GCR. First, we will develop a truncated version in which
the $Ap_i$'s are only orthogonal to the $m$ previous ones. This is dictated by practical
considerations, because keeping all $A p_i$ vectors may otherwise require too much memory.
Second, we will keep a set of vectors
for the $p_i$ and another set for the vectors $v_i \equiv A p_i$, for $i=1, \cdots, j$ at step $j$ to avoid unnecessary additional products of the matrix $A$ with vectors. The
truncated GCR (TCGR) is briefly summarized in Algorithm \ref{alg:tgcr}.
In the literature on iterative methods for linear systems, TGCR is also
known as ORTHOMIN, see, e.g.,  \cite[pp 195-196]{Saad-book2}.

  \begin{algorithm}[H]
    \centering
    \caption{TGCR(m)}\label{alg:tgcr}
    \begin{algorithmic}[1]
  \State \textbf{Input}: Matrix $A$, RHS $b$,
  initial  $x_0$. \\
  Set $r_0 \equiv b-Ax_0$; $v = A r_0$; 
  \State $v_0 = v/\| v \|$;   $p_0 = r_0 / \| v \|$; 
\For{$j=0,1,2,\cdots,$ Until convergence} 
\State  $\alpha_j = (r_j, v_j) $
\State $x_{j+1} = x_j + \alpha_j p_j$
\State $r_{j+1} = r_j - \alpha_j v_j$
\State $p = r_{j+1}$;  \quad  $ v = A p $;   \quad  and  \quad  $i_0 = \max(1,j-m+1)$  
\For{$i=i_0:j$} 
\State $\beta_{ij} :=  (v, Ap_i) $
\State $p := p - \beta_{ij} p_i$;
\State  $v := v - \beta_{ij} v_i$; 
\EndFor
\State $p_{j+1} :=p /\| v\|$ ; \qquad  $v_{j+1} :=v/\|v\|$ ; 
\EndFor
\end{algorithmic}
\end{algorithm}

With $m = \infty $ we obtain the non-restarted GCR method, which is equivalent
to the non-restarted (i.e., full) GMRES.  The purpose of Lines 8 to 14 is to compute the new
direction $p_{j+1}$ -- by ortho-normalizing the vector $Ar_{j+1}$ against all
previous $Ap_i$'s.
In fact the loop of  lines 9--13, implements a modified Gram-Schmidt procedure, which in exact
arithmetic amount simply to setting $p_{j+1}$ to
\eq{eq:equivAlg}
\beta_{j+1,j} p_{j+1} := r_{j+1} - \sum_{i=i_0}^j \beta_{ij} p_i \quad \mbox{where}\quad
\beta_{ij} = (Ar_{j+1}, A p_i) \ \mbox{for} \ i_0 \le i \le j. 
\en
In the above relation, $\beta_{j+1,j}$ is the scaling factor $\| v\|$ used to normalize
$p$ and $ v$ in Line~14. 
Then, $v_{j+1} \equiv A p_{j+1}  $ is computed accordingly as is reflected  in lines~12
and 14.
The update relation 
$A p_{j+1} = A r_{j+1} - \sum_{i=i_0,j} \beta_{ij}Ap_i$  (from Line 12) shows
that $A p_{j+1} \perp A p_i $ for $i=i_0, ...,j$.  In addition, it can
easily be shown that in this case ($m=\infty$) the residual vectors produced by the algorithm
are $A$-conjugate in that $(r_{j+1}, A r_i) = 0$ for $i\le j$.
Indeed, this requires a simple induction argument exploiting the  equality:
\[ 
  (r_{j+1}, A r_i) = (r_j -\alpha_j A p_j, A r_i) = (r_j , A r_i)  -\alpha_j (A p_j, A r_i) 
\]
and relation \nref{eq:equivAlg} which shows that $A r_{i} = \sum \beta_{k,i-1} A p_k $.



An important
consequence of this is that when the matrix $A$ is symmetric, then Algorithm
\ref{alg:tgcr} simplifies and leads to the Conjugate Residual algorithm.
Indeed, in this situation by exploiting the relation
$r_{i+1} = r_i - \alpha_i A p_i$, we can see that the scalar $\beta_{ij} $ in
Line~11 is
\[
  \beta_{ij} = (A r_{j+1}, A p_i) = \frac{1}{\alpha_i}
  (A r_{j+1}, r_i - r_{i+1}) = \frac{1}{\alpha_i}  =
  (r_{j+1}, A r_i - A r_{i+1}) 
\]
which is equal to zero for $i < j$. Therefore we need to orthogonalize
$Ar_{j+1}$ against vector $Ap_j$ only in the loop of lines 9 to 13.
This leads to big savings both in terms of memory and in computational costs.


The optimality of TGCR is proved in Theorem \ref{thm:tgcr}. 

\begin{theorem}
\label{thm:tgcr}
Let $r$ be the residual generated by the basic \methodName~, the following relations hold:
\begin{enumerate}

\item $\Span \{p_0, \cdots, p_{m-1} \} =
  \Span \{r_0, \cdots, A ^{m-1} r_0 \} \equiv K_m(r_0, A)$

\item If $m \ge j$,  the set of vectors $ \{A p_i \}_{i=1:j} $ is orthonormal.

\item More generally:  $ (A p_i, A p_j) = \delta_{ij}$ for
  $|i-j| \le m-1 $  

\item If $m \ge j$, then  $ \| b - A x_j \| = \min \{ \| b - A x \| \quad \vert \quad  \ x \ \in \
  x_0 + K_m(r_0,A) \}$

  \end{enumerate} 
\end{theorem}



  \subsection{The nonlinear case: nlTGCR}
  Assume now that we want to solve the nonlinear system of equations
  \eq{eq:Fx}
  F(x) = 0 . 
  \en
  Given an initial guess $x_0$, inexact Newton methods \cite{Dembo-al,Brown-Saad},
  compute a sequence of iterates   as follows
  \begin{align} 
 &      \mbox{Solve}  & J(x_j) \delta_j   &\approx -F(x_j) &  \label {eq:inex}\\
 &       \mbox{Set}    & x_{j+1}  & = x_j + \delta_j & \label {eq:updt}
  \end{align}  
  Here, $J(x_j)$ is the Jacobian of $F$ at the current iterate $x_j$.
  In \nref{eq:inex}  the system is solved inexactly, typically by some iterative method.
  Note that the right-hand side in the system is $-F(x_j)$ and this is also
  the residual for $x_j$, i.e., when $\delta_j = 0$. 
  Therefore, we will define the residual vector $r_j$  to  be $r_j = -F(x)$.

  If $P_j$ is the matrix whose columns contain the search directions $p_i$,
  then  we write the linear model used in inexact Newton methods as:
  \eq{eq:JP}  F(x_j + P_j y) \approx F(x_j) + [J] P_j y \quad
  \mbox{where} \quad  [J] P_j \equiv
  [ J(x_{i_0}) p_{i_0}, \cdots,  J(x_{j}) p_{j} ] = V_j , \en
  since $J$ is not the same for each iterate $x_i$.
  So the projection method that minimizes the norm
  $\| F(x_j) + [J] P_j y \| = \| F(x_j) + V_j y \| $ of the right-hand side
  determines $y$ in such a way that
  \eq{eq:opt} F(x_j) + V_j y \perp \Span
  \{V_j\} \ \rightarrow \ (V_j)^T[F(x_j) + V_j y] = 0 \ \rightarrow \ y = 
  V_j^T r_j \en 
    where it is assumed the the $v_i$'s are fully     orthogonal.
   Note that in the linear case, it can be shown that $V_j^T r_j$ has only one nonzero component when one assumes that the vectors $J p_i$ are fully orthogonal, i.e., that $i_0 =1$ always. 
   In the situation we have partial orthogonality ($i_0> 1$) -- one can solve
   the least-squares problem explicitly instead of exploiting orthogonality.

    
  
 The changes we need to make relative to Algorithm~\ref{alg:tgcr} are as
 follows.  First, any residual is now the negative of $F(x)$ so in Line~2
 $r_0 = - F(x_0)$ and Line~7 must be replaced by $r_{j+1} = - F(x_{j+1})$. In
 addition, we need to calculate the products $A r_0 $ and $A p$ in Line~2 and
 Line~8 respectively. Here $A$ is just the Jacobian $J(x_j)$ of $F$ at the
 current iterate which we denote by $J$ in the algorithm.  The most important
 change is in lines 5-6 where according to the above discussion $\alpha_j$ of
 Algorithm~\ref{alg:tgcr} is replaced by a vector $y_j$.

  %% In the linear case, these are based on Lemma~6.21 of  \cite{Saad-Book2}.
  
    \begin{algorithm}[H]
    \centering
    \caption{nlTGCR(m)}\label{alg:nltgcr}
    \begin{algorithmic}[1]
  \State \textbf{Input}: $F(x)$,   initial  $x_0$. \\
  Set $r_0 = - F(x_0)$.
  \State Compute  $v = J r_0$; \ (Use Frechet)
  \State $v_0 = v/ \| v \| $, $p_0 = r_0/ \| v \| $;
  \For{$j=0,1,2,\cdots,$ Until convergence} 
\State  $y_j = V_j^T r_j $ 
\State $x_{j+1} = x_j + P_j y_j$
\State $r_{j+1} = -F(x_{j+1}) $ 
\State Set: $p := r_{j+1}$; and $i_0 = \max(1,j-m+1)$
\State Compute $v =  J p$ (Use Frechet)
\For{$i=i_0:j$}
\State $\beta_{ij} :=  (v, v_i) $
\State $p := p - \beta_{ij} p_i$
\State $v := v - \beta_{ij} v_i$
\EndFor
\State $p_{j+1} :=p /\| v\|$ ; \qquad  $v_{j+1} :=v/\|v\|$ ; 
\EndFor
\end{algorithmic}
\end{algorithm}

 
nlTGCR(m) requires 2 function evaluations per step : one in Line 8 and the
other in Line~10.
In the situation when computing the Jacobian is inexpensive, then one can compute
$J p$ in Line~10 as a matrix-vector product and this will reduce the number of function
evaluations per step from 2 to 1. At a given step, nlTGCR(m) attempts to approximate a Newton step:
$  x_{j+1} = x_j + \delta $ where
$\delta $ is an approximate solution to $ J(x_j) \delta + F(x_j) = 0$.

We consider two possible versions of nlTGCR. In what follows we 
assume that all the $J p_i$'s are  computed exactly and that $m = \infty$.
\subsubsection{Analysis for the linearized update version} 


First, we consider a variant of the algorithm which we call
the ``linearized update version'' -- whereby 
 in Line~8 we update the
residual by using the linear model, namely, we replace Line~8 by

\bigskip
\hrule
\betab
\> 8a:  \>  $ r_{j+1} = r_j - V_j y_j$
\entab
\smallskip \hrule \bigskip


When $F$ is linear, then the residual at step $j+1$ becomes
$r_{j+1} = b - A(x_j + P_j y_j) = r_j - A P_j y_j $ and we recall that
$Ap_i$ is saved as $v_i$.
In this situation, it turns out that $y_j$ has only one nonzero component,
namely the last one.
Indeed, the optimality of the GCR/GMRES algorithm implies that at step $j$
the residual vector $r_j$ is orthogonal the $J K_{j-1}$ where $K_{j-1}$ is the
  $(j-1)$-st Krylov subspace. This implies that
  \[
    (r_j, J p_i) = 0, \quad \mbox{for}\quad i=0,\cdots, j-1
  \]
See also Lemma~6.21 in \cite{Saad-book2}.

Assume that we perform $k$ steps of the algorithm to produce $x_k$.
This means that Line~5 is replaced by
\texttt{``for $j = 0, 1, 2, \cdots, k$ do''}.
Then it is easy to see that the algorithm is exactly  equivalent to
an \emph{inexact Newton method} in which GMRES (or GCR) is invoked to solve the
Jacobian linear system - \cite{Brown-Saad}.
Indeed, in this situation Lines 4-15 of Algorithm~\ref{alg:tgcr} and Lines
5-17 of Algorithm~\ref{alg:nltgcr} are identical.
In other words, in Lines 5-17,
Algorithm~\ref{alg:nltgcr} is performing $k$ steps of
the GCR algorithm for solving the linear systems $F(x) + J P y = 0$.
In addition note that while the update is written in progressive form
as $x_{j+1} = x_j + \alpha_j p_j$, \emph{the right-hand side does
not change during the algorithm and it is equal to $r_0 = - F(x_0)$.
}
In effect $x_k$ is updated from $x_0$ by adding a vector from the Krylov subspace
or equivalently the span of $P_k$.

It was shown in \cite{Brown-Saad} that under mild conditions, the update to the
iterate is a descent direction. In addition, the article describes `global convergence
strategies' based on linesearch and trust-region techniques.
If we do not apply a global convergence strategy, then algorithm may have difficulties
converging.

\subsubsection{Analysis of the non-linear update version}
The linear-update  version of the algorithm discussed above can be unreliable if
a global convergence strategy, such as a trust-region technique, is not added.
Here we consider the `nonlinear-update version' as described in
Algorithm~\ref{alg:nltgcr}. This version explicitly enforces the
linear optimality condition of GCR, as represented by Equation~\nref{eq:opt}.

\paragraph{The  Inexact Newton viewpoint. \;}
What is remarkable is that while in the standard linear-update version
we minimize $\| F(x_0) + J(x_0) P y \|$, in the nonlinear update case, 
we minimize $\| F(x_j) + [J] P_j y \|$ where $x_j$ is now the most recent update,
where we recall our notation in \nref{eq:JP}. 

In the following we define $\delta_j = x_{j+1} - x_j = P y_j$.
Inexact Newton methods minimize $\| F(x_0) + J(x_0) P_j y \|$
over $y$  by using some iterative method and  enforcing a condition like
\[
  \| F(x_0) + J(x_0) P_j y \|  \le \eta  \| F(x_0) \|
\]
where $\eta < 1  $ is a paramater, see, e.g.,
\cite{Dembo-al,Brown-Saad, Brown-Saad2,Eisenstat-Walker94}.

In the new context we are trying to solve $F(x_j) + J(x_j) \delta = 0$  by
minimizing $ \| F(x_j) + [J] P_j y \| $.
Recall that by definition \nref{eq:JP} $[J] P_j$ should be interpreted
  as $[J] P_j \equiv V_j$.
Similarly to the
standard inexact Newton context, we could  also enforce the condition:
\eq{eq:eta2nd}
  \| F(x_j) + [J] P_j y \|  \le \eta  \| F(x_j) \| . 
  \en
  However, this would require a small modification to the scheme because
  as implemented in Algorithm~\ref{alg:nltgcr} $P_j$ is fixed and the solution
  obtained at this step may not necessarily satisfy \nref{eq:eta2nd} 

We can state the following simple results.



\begin{proposition}
%%  Let $m=\infty$ (full orthogonalization case).
  As defined in  Algorithm~\ref{alg:nltgcr}, $\delta_j $ minimizes
  $ \| F(x_j) + \delta \| $ over vectors of the form $\delta = V_j y$,
  where $y \ \in \ \RR^{n_j}$
  and $n_j = j-i_0+1$.
\end{proposition}

\begin{proof}
See above. 
\end{proof}

THE FOLLOWING NEEDS TO BE REDONE: 

\begin{proposition}
  Assume that  $J(x_j)$ is nonsingular and that $y_j \ne 0$. 
  Then $\delta_j = P_j y_j$ is a descent direction for the function $f = \half \| F(x) \|^2 $ at $x_j$.
\end{proposition}
\begin{proof}
  It was shown in \cite{Brown-Saad2} that a sufficient condition for $\delta$ to be a
  descent direction for $f$ is that $\| F(x_j) + J(x_j) \delta \| <  \| F(x_j) \|$.
  If $y_j \ne 0$ and $J(x_j)$ is nonsingular then
  $P_j y_j = \delta_j \ne 0$ -- (need to assume the $p_i$ independent)
  
  In addition, we have: 
  \begin{align*}
    \| F_j + [J] P_j y_j \|^2 = \| F_j + V_j y_j \|^2 = 
    &=     \| F_j\|^2 + 2 (F_j,V_j y_j) + \| V_j y_j \|^2 \\
    &=     \| F_j\|^2 + 2 (V_j^T F_j, y_j) + \| y_j \|^2 \\
    &=     \| F_j\|^2 - 2 (y_j, y_j) + \| y_j \|^2 \\
    &=     \| F_j\|^2 -  \| y_j \|^2 ,
  \end{align*}
  which proves the result.  Note thath we used the fact that $V_j$ is orthogonal
  so that $ \| V_j y_j \|^2 = \| y_j \|^2$ and the definition $y_j = - V^T F_j$.
\end{proof}

Since $\delta_j$ is a descent direction, we can use the same techniques used in inexact Newton
methods, see~\cite{Brown-Saad2}, to design global convergence strategies.
 
\paragraph{The Quasi-Newton viewpoint. \;}
It is also possible to view the algorithm from the alternative angle of
a Quasi-Newton approach  instead of  Inexact Newton.
In this viewpoint,  the inverse of the Jacobian
is approximated progressively. Because it is the inverse Jacobian that is
approximated, the method is akin to Broyden's second update method.

In our case, the approximate inverse Jacobian $G_j$ at step $j$ is equal to
\eq{eq:Gj}
G_{j} = P_j V_j^T .
\en 
If we apply this to the vector $v_j$ we get
$
  G_{j} v_j = P_j V_j^T v_j =  p_j =   \inv{J(x_j)} v_j .
$ 
So $G_j$ inverts $J(x_j)$ exactly when applied to $v_j$. It therefore satisfies 
the \emph{secant} equation (\cite[sec. 2.3]{FangSaad07}) 
\eq{eq:msecant1} 
  G_j v_j = p_j . 
  \en
This is the equivalent to the secant condition
$G_j \Delta f_j = \Delta x_j$ used in Broyden's second update method.
Broyden type-II methods replace
Newtons's iteration: $x_{j+1}  = x_j - \inv{Df(x_j)}  f_j$ with 
$     x_{j+1} = x_j - G_j f_j $  
  where $G_j $  approximates the inverse of the Jacobian $Df(x_j)$ at $x_j$
  by the  update formula $G_{j+1} = G_j + (\Delta x_j - G_j \Delta f_j) v_j^T $
  in which $v_j$ is defined in different ways see \cite{FangSaad07} for details. 


In addition, the update $G_j$ satisfies the `no-change' condition:
\eq{eq:msecant2} 
  G_j q = 0 \quad \forall q \perp v_j  .
  \en
  The usual no-change condition for secant methods is of the form
  $(G_j-G_{j-m}) q = 0 $ for $q \perp \Delta f_j$ which in our case
  would be 
  $(G_j-G_{j-m}) q = 0 $ for $q \perp \ v_j $.
  One can
  therefore consider that we are updating $G_{j-m} \equiv 0$.

\iffalse 
[TODO] It is possible to show that this matrix is the best approximation
to $J\inv$ that has the range $\Span\{ V_j \}$  ??

===========================  Addition
\fi 

It is also possible to find a link between the method proposed herein
and the Anderson acceleration reviewed in Section~\ref{sec:AA1},
by unraveling  a relation with multi-secant methods.
Note that equation~\nref{eq:msecant1} is satisfied for (at most) $m$ previous
instances of $j$, i.e., at step $j$ we have ($i_0$ defined in the algorithm)
$ 
  G_j v_i = p_i $ {for} $i=i_0, \cdots, j .  
$ 
  In other words we can also write
\eq{eq:msecant1M}
 G_j V_j = P_j   .   
  \en  
  This is similar to the multi-secant condition
  $ G_j {\cal F}_j ={\cal X}_j $ of Equation
  \nref{eq:mscond} -- see also
  equation (13) of \cite{FangSaad07} where   $  {\cal F}_j $
  and   $  {\cal X}_j $ are defined in \nref{eqn:dfdx}.
  In addition, we clearly also have a multi secant version of the no-change
  condition \nref{eq:msecant2}  seen above, which becomes: 
  \eq{eq:msecant2M}
  G_j q = 0  \quad \forall \quad q  \perp \Span\{ V_j \} .
  \en
  This is similar to the no-change condition represented by
  eq. (15) of  \cite{FangSaad07}, which stipulates that 
  $(G_j - G_{j-m}) q = 0$ for all $q$ orthogonal to the span of the
  subspace $\Span \{ {\cal F}_j \}$ mentioned above, provided we define
 $ G_{j-m}= 0$. 
 
 
 \begin{theorem}[Optimality of nltgcr(m) updates from Quasi-Newton Viewpoint]
 The matrix $G_j$ is the best approximation to the inverse Jacobi $\inv{J(x_i)}$ of $F(x)$ at $x_i$ among  all the matrices $G$ whose range $\operatorname{Range}(G) = \operatorname{Span}\{ V_j \}$. That is,
%  \begin{align}
%      \label{eq: Hessian-optimality}
%      G_j = \underset{\{G \in \mathbb{R}^{d\times d}| GV_j = P_j\}}{\operatorname{arg\min}} \norm{GJ(x_i) - I}_{\operatorname{Pro}(\operatorname{Span}\{ V_j \})} = \norm{P_{V_j}((G_j + \Delta)J(x_i) - I)}
%  \end{align}
\begin{align}
     \label{eq: Hessian-optimality}
     G_j = \underset{\{G \in \mathbb{R}^{d\times d}| GV_j = P_j\}}{\operatorname{arg\min}} \norm{GJ(x_i) - I}
 \end{align}
 where $P_{V_j} = V_j(V_j^{T}V_j)^{-1}V_j^{T} = V_jV_j^{T}$ is the orthogonal projection operator onto the space $\operatorname{Span}\{ V_j \})$.
 \end{theorem}

  \paragraph{Comparison with Anderson Acceleration}

\begin{wraptable}{r}{2.5cm}
 \begin{center}
 \begin{tabular}{c|c}
   AA         & nlTGCR  \\ \hline
   $\XX_j$    & $P_j$   \\
   $\FF_j$    & $V_j$ \\
   $\theta_j$ &  $- y_j$ \\
  \end{tabular}
  \end{center}
\end{wraptable}


Let us  set $\beta = 0$ in Anderson acceleration.
Without loss of generality  and in an effort  to simplify notation we also assume that $i_0 = 1$ each time.
 According to
 (\ref{eq:AA}--\ref{eq:thetaj}), the $j$-th iterate becomes simply
 $x_{j+1} = x_j - \FF_j \theta_j $ where
 $\theta_j$ is a vector that minimizes $\| f_j - \FF_j \theta \|$.
 For nlTGCR, we have $x_{j+1} = x_j + P_j y_j $
 where $y_j $ minimizes $ \| f_j + V_j y \| $. So this  is identical with
 Equation \nref{eq:AA} when $\beta = 0$  in which  $P_j \equiv \XX_j$,
 and $\FF_j$ is replaced by $V_j$.
 


  The most important relation for both cases is the multi-secant relation.
  For Anderson, we have
  \[ \FF_j = [f_1 - f_0, f_2 - f_1, \cdots, f_j - f_{j-1}] \quad
    \XX_j = [x_1 - x_0, x_2 - x_1, \cdots, x_j - x_{j-1}] \]
  and, with  $ G_{j-m} = 0 $,    the multi-secant matrix in \nref{eq:msec} becomes
  \eq{eq:AAb0}
    G_{j} = \XX_j  (\FF_j^T\FF_j)^{-1}\FF_j^T
  \en 
  which can be easily seen to minimizes $ \| G \|_F$ for matrices $G$ that satisfy
the multisecant condition $     G \FF_j = \XX_j $ 
  and the no-change condition
  $
    G_j^T (G_j  - G) = 0 . 
  $ 
\iffalse
  \begin{proof}
    Let $G$ a matrix as specfied above and set $\Delta = G_j - G$.
    Then
    \[ \| G \|_F^2 = \| G_j + \Delta \|^2 = \| G_j\|^2  + 2
      \underbrace{\Tr{G_j^T \Delta}}_{= 0}  + \|\Delta\|_F^2  \ge  \| G_j\|^2  . 
      \]
    \end{proof}
    \fi
    
    Consider now nlTGCR. If we set $\FF_j \equiv V_j $ and $\XX_j = P_j$ in Anderson,
    the multisecant matrix $G_j$ in \nref{eq:AAb0} simplifies to \nref{eq:msecant1M} -
    which also minimizes $\|G \|_F$ under the secant conditopn
    $G V_j = P_j$ and the no-change condition $G_j^T (G_j - G) = 0$.

    Therefore the two methods differ mainly in the way in which the sets
    $\FF_j / V_j$ ,  and $\XX_j / P_j $ are defined. Let us use the more general notation
    $V_j, P_j$ for the pair of subspaces. 

    In both cases, a vector $v_j$ is related to the corresponding $p_j$ by the fact that
    \eq{eq:ApproxNLT} v_j \approx J(x_j) p_j . \en
    In the case of nlTGCR this relation is explicitly enforced by
    a Frechet differentiation  (Line 10)-- before we perform an orthogonalization - which
    combines this vector with others -- without changing the span of the new $P_j$ (and also
    $V_j$). 

    In the case of AA, we have  $v_j = \Delta f_{j-1} = f_j - f_{j-1} $ and the relation exploited
    is that
    \eq{eq:ApproxAA}
    f_j \approx f_{j-1} + J(x_{j-1}) (x_j - x_{j-1}) \to
      \Delta f_{j-1} \approx J(x_{j-1}) \Delta  x_{j-1}
      \en
      
      However, relation \nref{eq:ApproxNLT} in nlTGMR is \emph{more accurate}- because we use an additional
      function evaluation to explicitly obtain  a more accurate approximation (ideally exact
      value)  for  $J(x_j) p_j$. In contrast when $x_j$ and $x_{j-1}$ are not close, then
      \nref{eq:ApproxAA} can be a very rough approximation. This is a key difference between the two
      methods. 

\iffalse        
      We also need to compare the two pairs of subspaces used: $P_j, V_j$ on the one hand
      and $\XX_j, \FF_j$ on the other.


 According to our earlier observation, $\XX_j$ is essentially the same as our $P_j$ - except for
 a scaling of the vectors. In addition, $\FF_j$ plays the role of our $V_j$ and
 what we call $y_j$ is the vector $\theta_j$ of AA. 
 If we had $\FF_j = V_j$ (up to scaling) the two methods would be identical.
 The only difference is the way in which the columns of $V_j$ are computed. It is important to note
 that 
\fi 
  


==> explainA.tex <==
\section{Additional Discussion}
\label{Sec:add}
{The method described in this paper mixes a number of
ideas coming from different horizons. Some of the high-level discussion provided below is
expanding further in later sections.}

{\paragraph{Linear case: TGCR}
Our initial idea was motivated by considering the linear case, in an attempt to  exploit
Conjugate-gradient like methods for solving a linear system $Ax=b$.
When $A$ is symmetric,  it is known
that it is possible to minimize the objective function $f(x) = \| b -Ax\|_2^2$
on the $k$-th Krylov subspace $\Span \{r_0, A r_0, \cdots, A^{k-1} r_0 \}$ by a
nice algorithm that uses a short-term recurrence. This
algorithm, called the Conjugate Residual algorithm, is quite similar to the
Conjugate Gradient but its residual vectors are conjugate (instead of being
orthogonal) and its search directions are $A^T A-$ conjugate (instead of being
$A$-conjugate). Its generalization to the nonsymmetric case, called the
Generalized Conjugate Residual method, is easy to obtain by enforcing these two
properties. Enforcing the $A^T A$ conjugacy of the $p_i$'s is the same as
enforcing the orthogonality of the vectors $A p_i$ and this is expensive when we
have many vectors. For this reason, practical versions of the algorithm are
\emph{truncated}, i.e., the orthogonalization is enforced against only a few
previous directions. The result is the TGCR(m) algorithm (Algorithm 1) -- which has been known since
the 1980s. It is
clear that \emph{we expect that when the matrix $A$ is nearly symmetric} TGCR(m)
will perform nearly as well as the full version GCR - because when $A$ is
symmetric, taking $m=1$ will yield full orthogonality of the $Ap_i$s (Theorem \ref{thm:appendTGCR}). }

{\paragraph{Nonlinear case: Newton Krylov} 
Suppose now that we have to solve the nonlinear system $F(x) = 0$ (in optimization 
$F$ is just the gradient of the objective function).
At this point, we may ask the question: why not just use an inexact Newton
method whereby the Jacobian system is 
solved with the \emph{linear} GCR or TGCR method? This is where Anderson acceleration
provides an interesting insight on some weaknesses of  Newton-Krylov method.
A Newton Krylov method generates a Krylov subspace $\Span \{r_0, J r_0, \cdots, J^k r_0 \}$
at a current iterate -- say $K = x_0$ -- (so $J \equiv J(x_0) \equiv DF(x_0)$) 
and tries to minimize
$F(x_0 + \delta)$ where $\delta \ \in \ K$, by exploiting the linear model:
$F(x_0 + \delta) \approx F(x_0) + J \delta$. If we generate a basis $V = [v_1, \cdots v_k]$ of $K$
and express $\delta $ as $\delta = V y$ then we would need to minimize
$\| F(x_0) + J V y \| $ which is a small least-squares problem. One usually adds to this
a global convergence strategies, e.g., a linesearch or a trust-region technique
to produce the next iterate $x_1$. 
The problem with this approach is this: \emph{the approximate solution obtained after
  $k$ steps of a Krylov subspace approach is based on the Jacobian at the initial point $x_0$.}
The intermediate calculation is entirely
linear and based on $J(x_0)$. It is not exploited in any way to produce
intermediate (nonlinear) iterates which in turn could be used to produce more
accurate information on some local Jacobian.  In contrast, a method like
Anderson acceleration (or in fact any of the secant or multisecant methods) will
do just this, i.e., it will tend to use information on the nonlinear mapping
near the most recent approximation to produce the new iterate.   This
distinction is rather important although if the problem is nearly linear, then
it could make little difference.}



{\paragraph{Nonlinear case: Anderson and nlTGCR}
Anderson acceleration can be viewed as a form of
Quasi-Newton method whereby the approximate inverse Jacobian is updated at each step
by using the collection of the previous iterates $x_k, x_{k-1}, \cdots x_{k-m+1}$ and the
corresponding function values $F_k, F_{k-1}, \cdots F_{k-m+1}$. To be more accurate it uses
the differences $\Delta x_j = x_{j+1} - x_j$ and the corresponding $\Delta F_j$ defined in the same way. 
Similarly to  Newton-Krylov, it generates
an approximation of the form $x_k + P y$ where $P$ is a basis of the subspace spanned
by the $\Delta x_j$'s. Notice how the update now is on $x_k$  the latest point generated.
The previous iterates are used to essentially provide
information on the nonlinear mapping and its differential. This information is constantly updated
using the most recent iterate. Note that this is informally stated: Anderson does not
formally get an approximation to the Jacobian. It is based implicitly on exploiting the relation 
$F(x_{j+1})- F(x_j) \approx J (x_{j+1}- x_j)  $. Herein lies a problem that nlTGCR aims at
correcting: this relation is only vaguely verified.  For example,  
\emph{if we take $J$ to be $J(x_j) $, the Jacobian at  $x_j$,  the resulting linear  model is
bound to be extremely inaccurate at the beginning of the iteration.} }

{In nlTGCR, we try to improve on the Newton-Krylov approach, since our starting point is
TGCR which is generalized to nonlinear problems. We also take the viewpoint of
improving on Anderson Acceleration or multisecant methods by not relying on the
approximation
$F(x_{j+1})- F(x_j) \approx J (x_{j+1}-x_j)  $ mentioned above. 
This is achieved by adopting the projection viewpoint. Instead of
minimizing $\| F(x_0) + J  P y\|$ as in the inexact Newton mode,  we would like to now minimize
$\| F(x_k) + J  P y\|$ where $x_k$ is the most recent iterate.
This initial idea leads to a difficulty since there is not one $J$ but 
several ones at previous points and a single one of them will not be satisfactory.
Thus, we have a few  directions $p_i$ just like the differences $\Delta x_i$ in Anderson,
\emph{but now each $p_i$ will lead to a $J(x_i) p_i$ which - unlike in AA - is accurately
  computed and then saved.}
This feature is what we believe makes a difference in the performance of the algorithm -- although
this is something that would be rather difficult to prove theoretically. }



==> rebuttal.tex <==
% \documentclass[a4paper,12pt]{article}
% \usepackage{xcolor}
% \begin{document}
% \title{nlTGCR Rebuttal}
% \date{\today}  
% \maketitle

Dear Area Chair,

Hope this message finds you well. We very much appreciate your time.

Following preliminary reviews to our paper, we addressed those questions and concerns posted by reviewers. But, we haven't heard back from them yet. Although I understand that you are very busy, I wish to express my gratitude for your understanding and your favorable communication to them. 

We also want to raise a concern regarding reviewer B5Ra (reviewer \#3), as the comments were either not applicable to our paper or were already discussed in the original submission. We feel that our work maybe punished due to the reviewer’s misunderstanding. Please see our response to reviewer 3 for more details.

Thanks again! 

Best,
Paper8730 Authors


We thank all reviewers for their time and valuable comments. We are happy that the reviewers find our algorithm exciting (R2, R4), theoretical results sound (R1, R2, R4), note that the paper is well-connected to existing literature (R1, R2, R4) and mention that the experiments in our work are successful (R1, R2, R4).

We would like to highlight three key points:

1. More explanation and discussion on proposed algorithms and theoretical results:

We appreciate reviewers' questions and suggestions about more discussion of our algorithm, which helps us improve our presentation. We have added more high-level clarifications and explanations of the algorithms. Also, we have added an extra discussion of the differences between the convergence results for linear and nonlinear problems. Please see our latest revision (Sec 3 and A.1).

2. More theoretical and numerical results to support the algorithm's advantages:
We provided a local convergence rate of nlTGCR in our revision (Theorem B.4 in our revision). In addition, we show that nlTGCR(1) (only takes one inner iteration) is analogous to inexact-Newton methods, whereas they take many more inner iterations (Sec 3.1 and Appendix A in our revision).  Although it is not the focus of our work given the 9-page limit, we tried our best to incorporate suggestions from R3 and R4 to make our paper even stronger. We provided 2 additional deep learning experiments (LSTM and ResNet) with multiple runs in our revision (Appendix C.4), which suggests the superiority of nlTGCR.

3. R3:

We respectfully disagree with your comment regarding the theoretical results of our work as well as the underlying intuition. We suspect this is due to a misinterpretation. Please see our reply below. 

We hope we have addressed most concerns through our response below and with the revision!


\section{reply to R1}
We greatly appreciate your time and remarks.  We understand your concerns about W1): The main theoretical results deserve better explanation and clarification. We found these questions great and important, so we have tried our best to improve our work by explaining and clarifying our theoretical results. In addition, we have added more experiments to demonstrate the usefulness of our algorithm in practice. We hope it helps you appreciate our result better:


\begin{enumerate}
    \item 
\textbf{Question:} 
In Thm 3.1, the paper shows linear convergence rate for linear problems then in Thm 3.3 the paper shows superlinear and quadratic convergence rate for non-linear problems. This is somehow counter-intuitive, in the sense that non-linear problems converge faster than linear problems. A thorough clarification on the result is required, especially in explaining why the superlinear and quadratic convergence rate fails for linear problems.
Upon my understanding, this is caused by the failure of some conditions imposed in Thm 3.3, in which case we need to discuss whether these conditions are vacuous or not. In particular, Thm3 impose a residual check condition to make sure the residual is bounded by the function value. \textcolor{red}{Is there any theoretical justification that such conditions will eventually be satisfied? In other words, can we guarantee that these conditions will happen? }The second convexity type condition is also not very clear to me, it somehow assumes the vector $\mathbf{P}_ny_n$ has a negative inner product with the gradient $\nabla\phi(x_n)$. \textcolor{red}{How can we guarantee such a condition with a universal parameter $\alpha$ and $\beta$?}

\textbf{Answer:}
    In short, there is no contradiction between the linear convergence of TGCR and superlinear(quadratic) convergence of nlTGCR. 
    For linear problems $Ax= b$ where $A$ is an SPD matrix. {The linear convergence rate proved in Thm 3.1 is an optimal upper bound that is the same with CG and full memory GMRES. It does not deny the chance that TGCR can achieve a superlinear convergence rate, like CG and GMRES. 
    In practice, the convergence of Krylov space methods may be superlinear, depending on the distribution of the spectrum of the matrix $A$ and the spectral distribution of the error.  This is saying that superlinear convergence of TGCR can be achieved by assuming a distribution of the spectrum of the matrix $A$ and the spectral distribution of the error, but not residual check.   It is also worth mentioning that the short-term recurrence of TGCR proved in Thm 3.1 does not necessarily require $A$ to be definite, while CG does. This claim is supported by Figure 1c when $A$ is symmetric indefinite. Thus, we believe TGCR(1) is an attractive algorithm for solving linear problems.
    }
    

    
    For solivng nonlinear problems, nlTGCR can be interpreted as an inexact Newton method. When equipped with the residual check, nlTGCR can achieve global convergence. If we further impose global line search techniques, nlTGCR can potentially achieve superlinear (quadratic) convergence locally since the approximation is so accurate that inexact Newton is close to Newton method in this case. %\textcolor{blue}{Huan: while this is more expensive to achieve for inexact newton methods, i.e., newton krylov with GMRES.}
    
      {Regarding the line search conditions, we admit these conditions may be restrictive though they are widely used in the convergence analysis of inexact Newton and quasi-Newton methods. Yet, we argue that the residual check can be done at no additional cost since this quantity is accessible at each step.}
      Though not discussed in detail in the paper, a realistic practical implementation should include global convergence strategies that can be borrowed from Inexact or quasi-Newton approaches. 
      If the residual check condition is not satisfied, we can then invoke these techniques, e.g., line-search or trust-region. Note that 
      another option that has been used in the literature is to \emph{apply a safeguarding step}, i.e., to restart the process when needed by taking the next iterate as the output of a vanilla fixed point iteration mapping -- see, e.g. Reference [42] of the paper.

    Regarding the condition with a universal parameter $\alpha$ and $\beta$: 
    In short, as long as the assumptions in Theorem 3.2 hold, the direction $P_ny_n$ will be a descent direction. This is shown in Theorem B.8 (B.10 in revision) in the appendix. The condition with a universal $\alpha$ and $\beta$ in Theorem 3.3 is only used to prove the superlinear and quadratic convergence which is discussed in detail in \cite{Brown-Saad}.

\item  From another perspective, the BFGS method can achieve superlinear and quadratic convergence rate but its limited memory variant L-BFGS only enjoys linear convergence rate. Hence it is a bit suspicious to me how the limited-variant of Conjugate Residual method can achieve superlinear convergence rate.

    Regarding the analog of our method to L-BFGS:
    We are glad you read closely and build a good connection. And we would like to clarify the difference between BFGS vs L-BFGS and nlTGCR(m) vs nlTGCR($\infty$). There cannot be any superlinear convergence unless the solvers are accurate enough - which is to say unless we use a large enough subspace each time. This is what inhibits superlinear convergence in L-BFGS. On the other hand, when we apply nlTGCR to solve $F(x)=0$ where $F$ is the gradient of some objective function $\phi:\mathbb{R}^n\rightarrow\mathbb{R}$ to be minimized. The Jacobian of $F$ becomes $\nabla^2 \phi$  the Hessian of $\phi$. Since Hessian is always symmetric,  the accuracy of nlTGCR(m) is close to that of nlTGCR($\infty$) in this case. Hence, nlTGCR(m) can produce very accurate solutions - hence making a superlinear convergence possible. 
We hope this clarifies the point you are making.  
%%Please let us know if you would like to have %%a further explanation on this response.
    \item 
    \textbf{Question}
    It is well known that Newton/Quasi-Newton method are sensitive to step sizes, which is why they usually have a line search to determine the step size. However, in the proposed algorithm, the step-size seems to be in closed form and we assume the residual check is satisfied. In my opinion, it would be more appropriate to allow line search to fulfill the residual check or the convexity type condition and prove that the line search can always be satisfied.
    
    \textbf{Answer}
    
    We totally agree with your claim and observation. We are sorry for this confusion. Theoretically, we have to use backtracking to make sure the residual check holds. Regarding the superlinear and global convergence, we mentioned in Theorem 3.3 that the Goldstein-Armijo conditions should be met. Numerically, we observe that our algorithm performs very well even without a line search for all experiments included in the paper. As a result, we ignored this detail to make the algorithm more understandable since there are so many technique subtleties. And we have added this back in our revision to improve the clarification. 
    
    \item  \textbf{Question:}
    The theoretical analysis seems not requiring non-expansiveness on the operator. If I read it correctly, it guarantees finding stationary points in non-convex optimization with the same rate. Please provide some clarification on this point.

    \textbf{Answer:}
    Thank you for pointing this out. In fact, the generalities in Theorem 3.2(3.3) are not for free. If the property of the function is not desirable (non-expansive/non-convex), it becomes more difficult to satisfy the assumptions. For example, in Theorem 3.2, the non-singularity and boundedness is required for $J(x)$. If the function does not satisfy the assumption, say, degenerate at a point, then the algorithm may not converge to a stationary point. 
\end{enumerate}

Again, we thank the reviewer for appreciating our contributions and asking great questions. These very detailed questions let us realize it is necessary to include more discussion. If there are any remaining questions/concerns, we would be grateful if the reviewers raise them so that we could further improve our work.

\section{Reply to R2}
We thank you for the detailed feedback and suggestions. We really appreciate you found our work to be well written and well structured. Your comments and additional reference improved our paper. 
\begin{enumerate}
    \item the description of the stochastic setting was lacking.

    We are aware the description of the stochastic setting is important and thanks for your understanding that we put them in the appendix due to the page limit. We promise that we will update the paper according to your suggestions in the camera-ready version should our paper be accepted.
    
    \item clarify the dimensions of $X_j$, $\bar F_j$ and the matrices in equation 2. Define what the 'differences' $\nabla x_i$ and $\nabla F_i$ are.

    We are sorry for the confusion and understand where it comes from.
    the dimension of $X_i$ adn $\bar F_i$ is n by m, where n is the parameter size and m is the table size. 
    Let's say $x_i$ is the current iterate, and $x_{i+1}$ is the coming iterate after a mapping $H$. $F_{i+1} = x_{i+1} - x_i$. Then we can define
    $\Delta x_i$ as $x_{i+1}-x_{i}$ and $\Delta F_i$ as $F_{i+1}-F_{i}$. 
    
    
\end{enumerate}

\section{Reply to R3}
Thanks for your comments! We believe our whole work has been misinterpreted. In this response, we hope to address your whole comment 
and explain the theoretical results of our work. 

\begin{enumerate}
    \item \textbf{Some theoretical results are reported for the exact and full-memory setting}
    
    We kindly disagree with this statement. We guess your misunderstanding might come from this sentence ``In what follows we assume that all the $Jp_i’s$ are computed exactly". This is how we attempt to approximate a Newton step and has nothing related to full memory or not. We do not assume full memory for our theoretical results. 
    
    \item \textbf{The algorithm description is densely packed with approximations and hand-waving arguments.} We have a different opinion on this comment. First of all, we don't see our algorithms are packed with approximations. The implementation strictly follows the algorithms presented in the paper. 
    We have also added an extra explanation of the proposed algorithm in the latest revision (A.1). 

    \item \textbf{Q1:} For example, the paper mentioned the issue of symmetry can be mitigated by exploiting near-symmetry assuming we are in the neighborhood of the solution. How is the closeness to the optimal solution handled when we are far from the solution? These issues are not further developed in the algorithm description. It is also not clear which steps in the algorithm exploit the symmetry.

    We kindly disagree with the remark and believe you misunderstood our algorithm and its assumption. In fact, 
    we are just saying when the iterate is very close to the solution, it will change very slowly, thus Hessian will also not change too much. When the iterates are far from the solution, we can still use the proposed method as it can be interpreted as an inexact Newton method. In Algorithm 2, the i loop (Lines 12-16) exploits the (near) symmetry. This is because as explained in the paper, when the problem is near symmetric, the vector $y_j$ in Line 6 has only a few large entries. Thus, we can use a small $m$ which corresponds to the number of large entries in $y_j$ in this case. In the extreme case, when the Jacobian is the same in a few iterations, $m$ can be taken as small as $1$. 
        

    \item \textbf{Q2:} the claim of reducing memory usage is not substantiated in the paper, neither theoretically nor empirically. It seems to me the proposed method also saves similar $m+1$ extra vectors $p_iv_i$ . Also, the proposed method requires more function evaluations per iteration.
    
    \textbf{Ans:} 
    Regarding `the claim of reducing memory usage is not substantiated in the paper, neither theoretically nor empirically.', 
    we kindly disagree with this remark as well. The claim of reducing memory usage is clearly reflected by the algorithm itself, which suggests using a small number of past iterates via exploiting the near symmetry. When the problem is linear and symmetric, we can take $m=1$. We also want to point out that in line 164 of our submission, we have already stated that the detailed complexity analysis is provided in Appendix A.2. Compared to the Truncated Anderson Acceleration or other extrapolation methods, TGCR and NLTGCR can use only the most recent iterate to achieve good performance. Compared to inexact Newton, the cost of nlTGCR(1) is similar to Newton-Krylov(1) methods with Hessain system being solved by one iteration of Krylov methods at each step. Although the memory usage is similar, nlTGCR(1) is more accurate because we are implicitly using a much larger space for solving Hessian system due to the near symmetry structure. From this viewpoint, we are using smaller memory since Newton-Krylov(k) needs to be used to achieve the same accuracy as nlTGCR(1) where $k > 1$.
    
    Regarding`It seems to me the proposed method also saves similar $m+1$ extra vectors $p_iv_i$.' Yes, it saves two tables of past iterates, which is the same as Anderson Acceleration, as shown in Sec 2.1. Thus, TGCR/nlTGCR(m) has the same memory cost as AA(m). However, we showed that our method  TGCR/nlTGCR(1)

    \item \textbf{Q:} The result in Theorem 3 needs a very strong assumption in each iteration? How can we know in the first place if the condition is satisfied? 
    
    \textbf{A:} We agree the assumptions are indeed strong. However, these assumptions are necessary for proving global convergence and they are relatively common assumptions that are widely used in the optimization field. Here we list several recent papers using similar assumptions: \cite{Brown-Saad,JunziBoyd20,inexactN,practicalIN,BFGS_e,hansasy,ouyangAA}.
    Generally, we don't know if these conditions will hold. In practice, it's possible to implement a line search strategy to guarantee these conditions. 

    \item How is the result in the theorem compared to a classic method like Gauss-Newton?
    
In nlTGCR, we try to improve on the Newton-Krylov framework, since our starting point is
TGCR which is generalized to nonlinear problems. We also take the viewpoint of
improving on Anderson Acceleration or multisecant methods by not relying on the
approximation
$F(x_{j+1})- F(x_j) \approx J (x_{j+1}-x_j)  $. 
This is achieved by adopting the projection viewpoint. Instead of
minimizing $\| F(x_0) + J  P y\|$ as in the inexact Newton mode,  we would like to now minimize
$\| F(x_k) + J  P y\|$ where $x_k$ is the most recent iterate.
This initial idea leads to a difficulty since there is not one $J$ but 
several ones at previous points and a single one of them will not be satisfactory.
Thus, we have a few  directions $p_i$ just like the differences $\Delta x_i$ in Anderson,
\emph{but now each $p_i$ will lead to a $J(x_i) p_i$ which - unlike in AA - is accurately
  computed and then saved.}
This feature is what we believe makes a difference in the performance of the algorithm -- although
this is something that would be rather difficult to prove theoretically. 

    
    
    \item \textbf{Q:} Where is the parameter m in the theorem?
    
    Although m does not appear explicitly in the theorem, it is hidden in the residual check. Note the larger the m is, the easier the residual check will be satisfied. To be more specific, as m increases, the subspace $[J]P_j$ is enlarged which means $\|F(x_j)+ [J]P_j\|$ will be smaller and the condition $\|F(x_j)+ [J]P_j\| \leq \eta_n \|F(x_j)\|$ is more likely to be satisfied.
    
    \item \textbf{Q:} It should be noted in the paper that Theorem 3.1 is well-known for Krylov subspace methods, especially conjugate gradient. 

    \textbf{A:} Theorem 3.1 contains two separate theoretical results (1) TGCR(m) is equivalent to TGCR(1) for symmetric matrix $A$; (2) the convergence rate of TGCR(1) when $A$ is SPD. We agree with the referee that this convergence rate is the same as that of CG but the short-term-recurrence property of TGCR proved in Theorem 3.1 is more general than that CG as $A$ only needs to be symmetric for TGCR. Thus, TGCR(1) is an attractive algorithm for solving linear problems.

    \item The problem is small, not the ones that can demonstrate the storage issue that the paper claims superiority. The experiments report only single runs; it would be more reliable to report statistical results.
    
    As per your request, we have added two additional deep learning experiments by comparing nlTGCR with Nesterov and Adam on LSTM and Resnet. We provide the results and experimental details in Appendix C.4 in our latest revision. The test performance of nlTGCR compared with other algorithms is given in the table below. We can observe that nlTGCR consistently outperforms baselines. In addition to adding more large-scale experiments, we have also updated results in our submission with error bars now to show robustness, figure 6-12 in the revision.
    
\begin{table}[h!]
\small
  \begin{center}
    \caption{Performance on deep learning experiments on test sets}
    \label{tab:resnetcifar}
    \begin{tabular}{l | c c c c} 
      Method & {Acc (MNIST)} &{Acc (CIFAR10)} & { RMSE (air passenger)} & { RMSE (shampoo)}\\
      \hline
      Nestrov & 98.98 $\pm$ .33 & 86.84 $\pm$ .47 & 0.106 $\pm$ .06 & 0.0437 $\pm$ .014 \\
      Adam & 99.15 $\pm$ .15 & 84.76 $\pm$ .46  & 0.019 $\pm$ .008 & 0.0612 $\pm$ .018\\
      nlTGCR(1) & \textbf{99.24 $\pm$ .13} & \textbf{87.79 $\pm$ .22} & \textbf{0.015 $\pm$ .005} & \textbf{0.0435 $\pm$ .009}\\
      \hline
    \end{tabular}
  \end{center}
\end{table}
\end{enumerate}
We hope our detailed response better explains the contributions of our work. We are eager to know if you have any concerns remaining; if your concerns have been clarified, we sincerely hope it helps you re-evaluate our paper.

\section{Reply to R4}
Thank you for your valuable comments. We greatly appreciate that you think the algorithm is interesting and the variant of GCR straightforward yet worth investigating. Below we address your concerns one by one.
\begin{enumerate}
    \item { I would have liked more experiments to support the algorithm's efficiency}
    
    We added a numerical comparison of nlTGCR(1) with Adam and Nesterov by training a neural network on the CIFAR 10 dataset. We provide the results and experimental details in Appendix XX in our latest revision. The performance of nlTGCR compared with other algorithms is given in the table below. We can observe that our results outperform baselines. In addition, nlTGCR has a smaller variance during training and this suggests the nlTGCR is attractive.
    
    \item {Suggestion: spend more time explaining algorithms 1 and 2}
    
\textbf{High-level  clarifications}
The method described in this paper mixes a number of
ideas coming from different horizons. Some of the high-level discussion provided below is
expanding further in the updated version.

\paragraph{Linear case: TGCR}
Our initial idea was motivated by considering the linear case, in an attempt to  exploit
Conjugate-gradient like methods for solving a linear system $Ax=b$.
When $A$ is symmetric,  it is known
that it is possible to minimize the objective function $f(x) = \| b -Ax\|_2^2$
on the $k$-th Krylov subspace $\Span \{r_0, A r_0, \cdots, A^{k-1} r_0 \}$ by a
nice algorithm that uses a short-term recurrence. This
algorithm, called the Conjugate Residual algorithm, is quite similar to the
Conjugate Gradient but its residual vectors are conjugate (instead of being
orthogonal) and its search directions are $A^T A-$ conjugate (instead of being
$A$-conjugate). Its generalization to the nonsymmetric case, called the
Generalized Conjugate Residual method, is easy to obtain by enforcing these two
properties. Enforcing the $A^T A$ conjugacy of the $p_i$'s is the same as
enforcing the orthogonality of the vectors $A p_i$ and this is expensive when we
have many vectors. For this reason, practical versions of the algorithm are
\emph{truncated}, i.e., the orthogonalization is enforced against only a few
previous directions. The result is the TGCR(m) algorithm (Algorithm 1). It is
clear that \emph{we expect that when the matrix $A$ is nearly symmetric} TGCR(m)
will perform nearly as well as the full version GCR - because when $A$ is
symmetric, taking $m=1$ will yield full orthogonality of the $Ap_i$'s (Theorem B.2). 

\paragraph{Nonlinear case: Newton Krylov} 
Suppose now that we have to solve the nonlinear system $F(x) = 0$ (in optimization 
$F$ is just the gradient of the objective function).
At this point, we may ask the question: why not just use an inexact Newton
method whereby the Jacobian system is 
solved with the \emph{linear} GCR or TGCR method? This is where Anderson acceleration
provides an interesting insight on some weaknesses of  Newton-Krylov method.
A Newton Krylov method generates a Krylov subspace $K = \Span \{r_0, J r_0, \cdots, J^k r_0 \}$
at a current iterate -- say $x_0$ -- (so $J \equiv J(x_0) \equiv DF(x_0)$) 
and tries to minimize
$F(x_0 + \delta)$ where $\delta \ \in \ K$, by exploiting the linear model:
$F(x_0 + \delta) \approx F(x_0) + J \delta$. If we generate a basis $V = [v_1, \cdots v_k]$ of $K$
and express $\delta $ as $\delta = V y$ then we would need to minimize
$\| F(x_0) + J V y \| $ which is a small least-squares problem. One usually adds to this
a global convergence strategies, e.g., a linesearch or a trust-region technique
to produce the next iterate $x_1$. 
The problem with this approach is this: \emph{the approximate solution obtained after
  $k$ steps of a Krylov subspace approach is based on the Jacobian at the initial point $x_0$.}
The intermediate calculation is entirely
linear and based on $J(x_0)$. It is not exploited in any way to produce
intermediate (nonlinear) iterates which in turn could be used to produce more
accurate information on some local Jacobian.  In contrast, a method like
Anderson acceleration (or in fact any of the secant or multisecant methods) will
do just this, i.e., it will tend to use information on the nonlinear mapping
near the most recent approximation to produce the new iterate.   This
distinction is rather important although if the problem is nearly linear, then
it could make little difference.



\paragraph{Nonlinear case: Anderson and nlTGCR}
Anderson acceleration can be viewed as a form of
Quasi-Newton method whereby the approximate inverse Jacobian is updated at each step
by using the collection of the previous iterates $x_k, x_{k-1}, \cdots x_{k-m+1}$ and the
corresponding function values $F_k, F_{k-1}, \cdots F_{k-m+1}$. To be more accurate it uses
the differences $\Delta x_j = x_{j+1} - x_j$ and the corresponding $\Delta F_j$ defined in the same way. 
Similarly to  Newton-Krylov, it generates
an approximation of the form $x_k + P y$ where $P$ is a basis of the subspace spanned
by the $\Delta x_j$'s. Notice how the update now is on $x_k$  the latest point generated.
The previous iterates are used to essentially provide
information on the nonlinear mapping and its differential. This information is constantly updated
using the most recent iterate. Note that this is informally stated: Anderson does not
formally get an approximation to the Jacobian. It is based implicitly on exploiting the relation 
$F(x_{j+1})- F(x_j) \approx J (x_{j+1}- x_j)  $. Herein lies a problem that nlTGCR aims at
correcting: this relation is only vaguely verified.  For example,  
\emph{if we take $J$ to be $J(x_j) $, the Jacobian at  $x_j$,  the resulting linear  model is
bound to be extremely inaccurate at the beginning of the iteration.} 

In nlTGCR, we try to improve on the Newton-Krylov approach, since our starting point is
TGCR which is generalized to nonlinear problems. We also take the viewpoint of
improving on Anderson Acceleration or multisecant methods by not relying on the
approximation
$F(x_{j+1})- F(x_j) \approx J (x_{j+1}-x_j)  $ mentioned above. 
This is achieved by adopting the projection viewpoint. Instead of
minimizing $\| F(x_0) + J  P y\|$ as in the inexact Newton mode,  we would like to now minimize
$\| F(x_k) + J  P y\|$ where $x_k$ is the most recent iterate.
This initial idea leads to a difficulty since there is not one $J$ but 
several ones at previous points and a single one of them will not be satisfactory.
Thus, we have a few  directions $p_i$ just like the differences $\Delta x_i$ in Anderson,
\emph{but now each $p_i$ will lead to a $J(x_i) p_i$ which - unlike in AA - is accurately
  computed and then saved.}
This feature is what we believe makes a difference in the performance of the algorithm -- although
this is something that would be rather difficult to prove theoretically. 


    
    \item \textbf{Q} No rate of convergence is presented, except for the quadratic case (which is trivial given the work on CR, equivalent to TGCR(1)). I know that proving convergence rates for nonlinear acceleration techniques is challenging, but local accelerated rates might be possible.
    
    We have incorporated your suggestions and added theoretical results. {If the Hessian near convergence is SPD, then the local convergence rate is the same as the rate of TGCR for solving a linear system, which is proved in Theorem 3.1. If the Hessian is indefinite, we have the local convergence rate $\frac{\left\|\mathbf{r}_{i}\right\|_{2}}{\|\mathbf{b}\|_{2}} \leq\left(\frac{\sqrt{\kappa_{+} \kappa_{-}}-1}{\sqrt{\kappa_{+} \kappa_{-}}+1}\right)^{\lfloor i / 2\rfloor}$
where $\lfloor i/ 2\rfloor$ means to round $i / 2$ down to the nearest integer. Here, we divide its eigenvalues of $A$ into positive and negative sets $\Lambda_{+}$and $\Lambda_{-}$, and define
$$
\kappa_{+}=\frac{\max _{\lambda \in \Lambda_{+}}|\lambda|}{\min _{\lambda \in \Lambda_{+}}|\lambda|}, \quad \kappa_{-}=\frac{\max _{\lambda \in \Lambda-\Lambda}|\lambda|}{\min _{\lambda \in \Lambda_{-}}|\lambda|}
$$
}  Please see Appendix B.3 in our revision. This rate is not difficult to obtain. We promise that we will update the paper according to your suggestions in the camera-ready version should our paper be accepted. 
    
    
    
    \item \textbf{Q} In addition to the previous point, it seems that the authors rely heavily on the residual check to ensure convergence. I understand that a nonlinear acceleration algorithm might requires safeguard steps to prevent them from diverging. However, the theorems that show convergence and superlinear convergence are somehow generic. For instance, the proof for superlinear convergence (paper's appendix on line 615) reads: "The following superlinear and quadratic convergence result can be derived similar to Theorem 3.15 in [40]."

    We appreciate you understand that a nonlinear acceleration algorithm might require safeguard steps to prevent them from diverging. We are aware our theoretical results leverage some existing works. However, this is because we show that the proposed algorithm, as an extension of Newton Krylov methods, is closely related to existing literature. For example, to give more valuable insights and novel results, we show that nlTGCR  is analogous to inexact-Newton methods, whereas the latter ones take many more inner iterations of Krylov methods.
    {Yet, we argue that the residual check can be done at no additional cost since this quantity is accessible at each step.} Though not discussed in detail in the paper, a realistic practical implementation should include global convergence strategies that can be borrowed from Inexact or quasi-Newton approaches. If the residual check condition is not satisfied, we can then invoke these techniques, e.g., line-search or trust-region. Note that another option that has been used in the literature is to \emph{apply a safeguarding step}, i.e., to restart the process when needed by taking the next iterate as the output of a vanilla fixed point iteration mapping -- see, e.g. Reference [42] of the paper.
    

\end{enumerate}

Again, we thank the reviewer for appreciating our algorithm and asking great questions. We have incorporated suggestions by adding new theoretical results (Appendix B.4) as well as our additional large experiments (Appendix C.4.) We'd like to get in touch with you again to know if we clarified your concerns and questions.
\bibliographystyle{unsrt}  %%%% remove when doing b1 -- b2. 
\bibliography{strings,eig,saad,local,local1,msecant,accelbib}
\end{document}

Thanks for your comments! We believe our whole work has been misinterpreted. In this response, we hope to address your whole comment and explain the theoretical results of our work. 

### 1, Some theoretical results are reported for the exact and full-memory setting
    
* We kindly disagree with this statement. We guess your misunderstanding might come from this sentence ``In what follows we assume that all the $Jp_i’s$ are computed exactly". This is how we attempt to approximate a Newton step and has nothing related to full memory or not. We do not assume full memory for our theoretical results. 
    
### 2, The algorithm description is densely packed with approximations and hand-waving arguments.

* We have a different opinion on this comment. First of all, we don't see our algorithms are packed with approximations. The implementation strictly follows the algorithms presented in the paper. We have also added an extra explanation of the proposed algorithm in the latest revision (A.1). 

### 3, For example, the paper mentioned the issue of symmetry can be mitigated by exploiting near-symmetry assuming we are in the neighborhood of the solution. How is the closeness to the optimal solution handled when we are far from the solution? These issues are not further developed in the algorithm description. It is also not clear which steps in the algorithm exploit the symmetry.

* We kindly disagree with the remark. In fact, we are just saying when the iterate is very close to the solution, it will change very slowly, thus Hessian will also not change too much. When the iterates are far from the solution, we can still use the proposed method as it can be interpreted as an inexact Newton method. In Algorithm 2, the i loop (Lines 12-16) exploits the (near) symmetry. This is because as explained in the paper, when the problem is near symmetric, the vector $y_j$ in Line 6 has only a few large entries. Thus, we can use a small $m$ which corresponds to the number of large entries in $y_j$ in this case. In the extreme case, when the Jacobian is the same in a few iterations, $m$ can be taken as small as $1$. 
        
### 4, the claim of reducing memory usage is not substantiated in the paper, neither theoretically nor empirically. It seems to me the proposed method also saves similar $m+1$ extra vectors $p_iv_i$ . Also, the proposed method requires more function evaluations per iteration.

* Regarding “the claim of reducing memory usage is not substantiated in the paper, neither theoretically nor empirically.”,  we disagree with this comment as well. The claim of reducing memory usage is clearly reflected by the algorithm itself, which suggests using a small number of past iterates via exploiting the near symmetry. When the problem is linear and symmetric, we can take $m=1$. We also want to point out that in line 164 of our submission, we have already stated that the detailed complexity analysis is provided in Appendix A.2. Compared to the Truncated Anderson Acceleration or other extrapolation methods, TGCR and NLTGCR can use only the most recent iterate to achieve good performance. Compared to inexact Newton, the cost of nlTGCR(1) is similar to Newton-Krylov(1) methods with Hessain system being solved by one iteration of Krylov methods at each step. Although the memory usage is similar, nlTGCR(1) is more accurate because we are implicitly using a much larger space for solving Hessian system due to the near symmetry structure. From this viewpoint, we are using smaller memory since Newton-Krylov(k) needs to be used to achieve the same accuracy as nlTGCR(1) where $k > 1$.
    
* Regarding “It seems to me the proposed method also saves similar $m+1$ extra vectors $p_iv_i$”. Yes, it saves two tables of past iterates, which is the same as Anderson Acceleration, as shown in Sec 2.1. Thus, TGCR/nlTGCR(m) has the same memory cost as AA(m). However, we showed that our method  TGCR/nlTGCR(1) outperforms AA(m>1), which suggest our algorithm is superior to AA.

* Regarding `the proposed method requires more function evaluations per iteration.', 
